DomainSum: A Hierarchical Benchmark for Fine-Grained Domain Shift in Abstractive Text Summarization

Most research on abstractive summarization focuses on single-domain applications, often neglecting how domain shifts between documents affect performance and the generalization ability of summarization models. To address this issue, we introduce DomainSum, a hierarchical benchmark designed to capture fine-grained domain shifts in abstractive summarization. We categorize these shifts into three levels: genre, style, and topic, and demonstrate through comprehensive benchmark analysis that they follow a hierarchical structure. Furthermore, we evaluate the domain generalization capabilities of commonly used pre-trained language models (PLMs) and large language models (LLMs) in in-domain and cross-domain settings.

==> tables/genre_result.tex <==


% \begin{table*}[t!]
% \centering
% \setlength{\tabcolsep}{3pt}

% \resizebox{.99\textwidth}{!}{
% \begin{tabular}{l| cc|  cc| cc| cc| cc }
%     \toprule
%     \multirow{2}{*}{Model} & \multicolumn{2}{c|}{\textbf{CNN/DM}} & \multicolumn{2}{c|}{\textbf{PubMed}} & \multicolumn{2}{c|}{\textbf{Reddit}} & \multicolumn{2}{c|}{\textbf{SAMSum}} & \multicolumn{2}{c}{\textbf{WikiHow}}   \\
%      & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore   \\
    
% \midrule
% \multicolumn{11}{c}{Zero-shot Setting (Two-shot Setting)} \\
% \midrule
    
% GPT-4o mini
% & \cellcolor{red!00}24.78 (-0.07) & \cellcolor{red!12}87.43 (+0.06) & \cellcolor{red!0}20.69 (+0.33) & \cellcolor{red!24}83.60 (+0.14) 
% & \cellcolor{red!00}10.91 (+5.20) & \cellcolor{red!00}81.48 (+1.58) & \cellcolor{red!00}25.01 (+4.83) & \cellcolor{red!12}89.34 (+1.08) 
% & \cellcolor{red!00}15.27 (+3.39) & \cellcolor{red!00}83.20 (+1.27)
% \\
% Mistral 7b
% & \cellcolor{red!00}25.82 (-0.65) & \cellcolor{red!12}87.43 (-0.10) & \cellcolor{red!24}22.06 (-0.59) & \cellcolor{red!00}83.49 (+0.28)
% & \cellcolor{red!00}10.72 (+2.68) & \cellcolor{red!00}81.36 (+0.91) & \cellcolor{red!00}23.76 (+4.44) & \cellcolor{red!00}89.10 (+0.94) 
% & \cellcolor{red!00}15.29 (+1.93) & \cellcolor{red!00}83.09 (+0.80) 
% \\
% Gemma1.1 7b
% & \cellcolor{red!00}23.68 (+0.66) & \cellcolor{red!00}86.28 (+0.28) & \cellcolor{red!00}20.74 (-1.21) & \cellcolor{red!00}83.25 (+0.14) 
% & \cellcolor{red!00}11.50 (-0.02) & \cellcolor{red!12}81.72 (+0.01) & \cellcolor{red!00}23.26 (+2.92) & \cellcolor{red!00}88.51 (+1.33) 
% & \cellcolor{red!00}16.09 (+0.66) & \cellcolor{red!00}82.72 (+0.47) 
% \\
% Llama3.1 8b
% & \cellcolor{red!24}26.02 (-0.80) & \cellcolor{red!24}87.46 (+0.14) & \cellcolor{red!0}21.07 (+1.54) & \cellcolor{red!12}83.54 (+0.18)
% & \cellcolor{red!12}11.83 (+3.82) & \cellcolor{red!24}81.81 (+1.07) & \cellcolor{red!24}26.11 (+5.05) & \cellcolor{red!24}89.61 (+0.84)
% & \cellcolor{red!12}16.75 (+1.69) & \cellcolor{red!12}83.21 (+0.71)
% \\
% Llama3.1 70b
% & \cellcolor{red!12}25.87 (-0.13) & \cellcolor{red!00}87.11 (-2.08) & \cellcolor{red!12}21.71 (+1.85) & \cellcolor{red!00}83.48 (-7.55)
% & \cellcolor{red!24}11.99 (+4.90) & \cellcolor{red!00}80.59 (+1.89) & \cellcolor{red!12}25.48 (+4.69) & \cellcolor{red!00}88.92 (+1.40)
% & \cellcolor{red!24}17.05 (+2.93) & \cellcolor{red!24}83.31 (+0.70)
% \\

    
%     \midrule
%     \multicolumn{11}{c}{Fine-tuning Setting} \\
%     \midrule
    
%     BART
%     & \cellcolor{red!24}28.43 & \cellcolor{red!24}87.72 
%     & \cellcolor{red!00}20.70 & \cellcolor{red!00}84.05 
%     & \cellcolor{red!24}20.86 & \cellcolor{red!24}87.46
%     & \cellcolor{red!24}37.61 & \cellcolor{red!24}91.56 
%     & \cellcolor{red!24}24.73 & \cellcolor{red!24}87.62 
%     \\
%     PEGASUS-X
%     & \cellcolor{red!00}25.54 & \cellcolor{red!00}86.73 
%     & \cellcolor{red!00}21.31 & \cellcolor{red!00}83.38 
%     & \cellcolor{red!00}15.74 & \cellcolor{red!00}85.37 
%     & \cellcolor{red!00}31.54 & \cellcolor{red!00}90.40 
%     & \cellcolor{red!00}16.75 & \cellcolor{red!00}83.08 
%     \\
%     Llama3.1 8b
%     & \cellcolor{red!00}25.81 & \cellcolor{red!00}86.91 
%     & \cellcolor{red!24}24.10 & \cellcolor{red!24}84.44 
%     & \cellcolor{red!00}13.31 & \cellcolor{red!00}79.69 
%     & \cellcolor{red!00}17.67 & \cellcolor{red!00}87.29 
%     & \cellcolor{red!00}19.78 & \cellcolor{red!00}83.53 
%     \\
    
  

%     \bottomrule

% \end{tabular}}
% \caption{Model performance based on genre shift across five datasets, with evaluation metrics including BERTScore F1 and the geometric mean of ROUGE-1/2/L (ROUGE). Parenthetical values represent the performance gains or losses observed when comparing two-shot prompting to zero-shot prompting.}
% \label{tab:1}
% % \vspace{-1em}
% \end{table*}








\begin{table*}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{.99\textwidth}{!}{
\begin{tabular}{l| cc|  cc| cc| cc| cc }
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{2}{c|}{\textbf{CNN/DM}} & \multicolumn{2}{c|}{\textbf{Pubmed}} & \multicolumn{2}{c|}{\textbf{Reddit}} & \multicolumn{2}{c|}{\textbf{SamSum}} & \multicolumn{2}{c}{\textbf{WikiHow}}   \\
     & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore   \\
    
    \midrule
    \multicolumn{11}{c}{Zero-shot Setting} \\
    \midrule
    
        
    GPT-4o mini
    & \cellcolor{red!00}24.78 & \cellcolor{red!12}87.43 & \cellcolor{red!0}20.69 & \cellcolor{red!24}83.60 
    & \cellcolor{red!00}10.91 & \cellcolor{red!00}81.48 & \cellcolor{red!00}25.01 & \cellcolor{red!12}89.34 
    & \cellcolor{red!00}15.27 & \cellcolor{red!00}83.20
    \\
    Mistral 7b
    & \cellcolor{red!00}25.82 & \cellcolor{red!12}87.43 & \cellcolor{red!24}22.06 & \cellcolor{red!00}83.49 
    & \cellcolor{red!00}10.72 & \cellcolor{red!00}81.36 & \cellcolor{red!00}23.76 & \cellcolor{red!00}89.10 
    & \cellcolor{red!00}15.29 & \cellcolor{red!00}83.09 
    \\
    Gemma1.1 7b
    & \cellcolor{red!00}23.68 & \cellcolor{red!00}86.28 
    & \cellcolor{red!00}20.74 & \cellcolor{red!00}83.25 
    & \cellcolor{red!00}11.50 & \cellcolor{red!12}81.72
    & \cellcolor{red!00}23.26 & \cellcolor{red!00}88.51 
    & \cellcolor{red!00}16.09 & \cellcolor{red!00}82.72 
    \\
    Llama3.1 8b
    & \cellcolor{red!24}26.02 & \cellcolor{red!24}87.46 & \cellcolor{red!0}21.07 & \cellcolor{red!12}83.54 
    & \cellcolor{red!12}11.83 & \cellcolor{red!24}81.81 & \cellcolor{red!24}26.11 & \cellcolor{red!24}89.61 
    & \cellcolor{red!12}16.75 & \cellcolor{red!12}83.21 
    \\
    Llama3.1 70b
    & \cellcolor{red!12}25.87 & \cellcolor{red!00}87.11 & \cellcolor{red!12}21.71 & \cellcolor{red!00}83.48 
    & \cellcolor{red!24}11.99 & \cellcolor{red!00}80.59 & \cellcolor{red!12}25.48 & \cellcolor{red!00}88.92 
    & \cellcolor{red!24}17.05 & \cellcolor{red!24}83.31
    \\
    
    


    \midrule
    \multicolumn{11}{c}{Two-shot Setting} \\
    \midrule
    GPT-4o mini
    & \cellcolor{red!00}24.71 & \cellcolor{red!12}87.49 
    & \cellcolor{red!00}21.02 & \cellcolor{red!12}83.74 
    & \cellcolor{red!12}16.11 & \cellcolor{red!24}83.06 
    & \cellcolor{red!00}29.84 & \cellcolor{red!12}90.42 
    & \cellcolor{red!12}18.66 & \cellcolor{red!24}84.47 
    \\
    Mistral 7b
    & \cellcolor{red!00}25.17 & \cellcolor{red!00}87.33 
    & \cellcolor{red!24}22.65 & \cellcolor{red!24}83.77 
    & \cellcolor{red!00}13.40 & \cellcolor{red!00}82.27 
    & \cellcolor{red!00}28.20 & \cellcolor{red!00}90.04 
    & \cellcolor{red!00}17.22 & \cellcolor{red!00}83.89 
    \\
    Gemma1.1 7b
    & \cellcolor{red!00}23.02 & \cellcolor{red!00}86.56
    & \cellcolor{red!00}19.53 & \cellcolor{red!00}83.39 
    & \cellcolor{red!00}11.48 & \cellcolor{red!00}81.73 
    & \cellcolor{red!00}26.18 & \cellcolor{red!00}89.84 
    & \cellcolor{red!00}16.75 & \cellcolor{red!00}83.19 
    \\
    Llama3.1 8b
    & \cellcolor{red!24}26.82 & \cellcolor{red!24}87.60 
    & \cellcolor{red!12}22.61 & \cellcolor{red!00}83.72 
    & \cellcolor{red!00}15.65 & \cellcolor{red!12}82.74 
    & \cellcolor{red!24}31.16 & \cellcolor{red!24}90.45 
    & \cellcolor{red!00}18.44 & \cellcolor{red!00}83.92 
    \\
    Llama3.1 70b
    & \cellcolor{red!12}25.74 & \cellcolor{red!00}85.03 
    & \cellcolor{red!00}19.86 & \cellcolor{red!00}75.93 
    & \cellcolor{red!24}16.89 & \cellcolor{red!00}82.48 
    & \cellcolor{red!12}30.17 & \cellcolor{red!00}86.32 
    & \cellcolor{red!24}19.98 & \cellcolor{red!12}84.01 
    \\
    
    \midrule
    \multicolumn{11}{c}{Fine-tuning Setting} \\
    \midrule
    
    BART
    & \cellcolor{red!24}28.43 & \cellcolor{red!24}87.72 
    & \cellcolor{red!00}20.70 & \cellcolor{red!00}84.05 
    & \cellcolor{red!24}20.86 & \cellcolor{red!24}87.46
    & \cellcolor{red!24}37.61 & \cellcolor{red!24}91.56 
    & \cellcolor{red!24}24.73 & \cellcolor{red!24}87.62 
    \\
    PEGASUS-X
    & \cellcolor{red!00}25.54 & \cellcolor{red!00}86.73 
    & \cellcolor{red!00}21.31 & \cellcolor{red!00}83.38 
    & \cellcolor{red!00}15.74 & \cellcolor{red!00}85.37 
    & \cellcolor{red!00}31.54 & \cellcolor{red!00}90.40 
    & \cellcolor{red!00}16.75 & \cellcolor{red!00}83.08 
    \\
    Llama3.1 8b
    & \cellcolor{red!00}25.81 & \cellcolor{red!00}86.91 
    & \cellcolor{red!24}24.10 & \cellcolor{red!24}84.44 
    & \cellcolor{red!00}13.31 & \cellcolor{red!00}79.69 
    & \cellcolor{red!00}17.67 & \cellcolor{red!00}87.29 
    & \cellcolor{red!00}19.78 & \cellcolor{red!00}83.53 
    \\
    
  

    \bottomrule

\end{tabular}}
\caption{Experimental results based on Genre.}
\label{tab:1}
% \vspace{-1em}
\end{table*}

==> tables/style_result.tex <==

% \begin{table*}[t!]
% \centering
% \setlength{\tabcolsep}{3pt}
% \resizebox{.99\textwidth}{!}{
% \begin{tabular}{l| cc|  cc| cc| cc| cc }
%     \toprule
%     \multirow{2}{*}{Model} & \multicolumn{2}{c|}{\textbf{CNN}} & \multicolumn{2}{c|}{\textbf{Fox}} & \multicolumn{2}{c|}{\textbf{NYDaily}} & \multicolumn{2}{c|}{\textbf{NYTimes}} & \multicolumn{2}{c}{\textbf{WaPo}}   \\
%      & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore   \\
    
%     \midrule
% \multicolumn{11}{c}{Zero-shot Setting (Two-shot Setting)} \\
%     \midrule
        
%     GPT-4o mini
%     & \cellcolor{red!00}16.76 (+0.11) & \cellcolor{red!12}84.58 (+0.11) & \cellcolor{red!0}19.06 (-0.20) & \cellcolor{red!12}85.27 (+0.17) 
%     & \cellcolor{red!00}20.80 (+0.05) & \cellcolor{red!12}85.19 (+0.34) & \cellcolor{red!00}15.37 (-0.52) & \cellcolor{red!12}84.32 (+0.16) 
%     & \cellcolor{red!00}11.33 (+0.10) & \cellcolor{red!24}83.52 (+0.18)
%     \\
%     Mistral 7b
%     & \cellcolor{red!24}18.18 (-0.01) & \cellcolor{red!24}84.64 (-0.13) & \cellcolor{red!24}21.21 (-0.30) & \cellcolor{red!24}85.42 (+0.04)
%     & \cellcolor{red!24}22.52 (-0.40) & \cellcolor{red!24}85.33 (-0.02) & \cellcolor{red!24}16.86 (+0.04) & \cellcolor{red!24}84.45 (+0.05) 
%     & \cellcolor{red!24}12.35 (+0.04) & \cellcolor{red!24}83.52 (+0.11) 
%     \\
%     Gemma1.1 7b
%     & \cellcolor{red!00}15.94 (+0.52) & \cellcolor{red!00}82.85 (+0.34) & \cellcolor{red!00}18.92 (-0.20) & \cellcolor{red!00}84.47 (+0.47) 
%     & \cellcolor{red!00}20.19 (+0.35) & \cellcolor{red!00}84.51 (-0.23) & \cellcolor{red!00}14.93 (-0.46) & \cellcolor{red!00}83.32 (+0.41) 
%     & \cellcolor{red!00}10.89 (+0.22) & \cellcolor{red!00}81.51 (+0.70) 
%     \\
%     Llama3.1 8b
%     & \cellcolor{red!12}17.46 (+1.68) & \cellcolor{red!00}83.85 (-0.08) & \cellcolor{red!12}19.95 (+2.75) & \cellcolor{red!00}85.17 (+0.42)
%     & \cellcolor{red!12}21.30 (+2.83) & \cellcolor{red!00}85.06 (+0.37) & \cellcolor{red!12}16.19 (+0.41) & \cellcolor{red!00}84.19 (-0.03) 
%     & \cellcolor{red!12}11.75 (+0.71) & \cellcolor{red!12}82.31 (+0.40)
%     \\
%     Llama3.1 70b
%     & \cellcolor{red!00}17.06 (+3.63) & \cellcolor{red!00}83.48 (-3.63) & \cellcolor{red!00}19.24 (+6.96) & \cellcolor{red!00}83.30 (+2.13)
%     & \cellcolor{red!0}20.24 (+3.49) & \cellcolor{red!00}81.52 (-1.22) & \cellcolor{red!00}15.77 (+2.45) & \cellcolor{red!00}81.67 (+1.93)
%     & \cellcolor{red!00}11.60 (+1.85) & \cellcolor{red!00}78.78 (+4.09)
%     \\


    
    
%     \midrule
%     \multicolumn{11}{c}{Fine-tuning Setting} \\
%     \midrule
    
%     BART
%     & \cellcolor{red!24}42.02 & \cellcolor{red!24}89.44 
%     & \cellcolor{red!24}55.05 & \cellcolor{red!24}91.55 
%     & \cellcolor{red!24}53.84 & \cellcolor{red!24}91.06 
%     & \cellcolor{red!24}25.38 & \cellcolor{red!24}86.81 
%     & \cellcolor{red!24}20.05 & \cellcolor{red!24}85.58 
%     \\
%     PEGASUS-X
%     & \cellcolor{red!00}38.20 & \cellcolor{red!00}88.16 
%     & \cellcolor{red!00}54.58 & \cellcolor{red!00}91.34 
%     & \cellcolor{red!00}49.45 & \cellcolor{red!00}90.33 
%     & \cellcolor{red!00}23.62 & \cellcolor{red!00}85.82 
%     & \cellcolor{red!00}18.34 & \cellcolor{red!00}84.39 
%     \\
%     Llama3.1 8b
%     & \cellcolor{red!00}20.55 & \cellcolor{red!00}85.27 
%     & \cellcolor{red!00}29.20 & \cellcolor{red!00}86.84 
%     & \cellcolor{red!00}33.91 & \cellcolor{red!00}87.70 
%     & \cellcolor{red!00}16.33 & \cellcolor{red!00}83.60 
%     & \cellcolor{red!00}10.66 & \cellcolor{red!00}82.70 
%     \\
    
  

%     \bottomrule

% \end{tabular}}
% \caption{Model performance based on style shift across five datasets, with evaluation metrics including BERTScore F1 and the geometric mean of ROUGE-1/2/L (ROUGE). Parenthetical values represent the performance gains or losses observed when comparing two-shot prompting to zero-shot prompting.}
% \label{tab:2}
% % \vspace{-1em}
% \end{table*}

\begin{table*}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{.99\textwidth}{!}{
\begin{tabular}{l| cc|  cc| cc| cc| cc }
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{2}{c|}{\textbf{CNN}} & \multicolumn{2}{c|}{\textbf{Fox}} & \multicolumn{2}{c|}{\textbf{NYDaily}} & \multicolumn{2}{c|}{\textbf{NYTimes}} & \multicolumn{2}{c}{\textbf{WaPo}}   \\
     & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore   \\
    
    \midrule
    \multicolumn{11}{c}{Zero-shot Setting} \\
    \midrule
        
    GPT-4o mini
    & \cellcolor{red!00}16.76 & \cellcolor{red!12}84.58 & \cellcolor{red!0}19.06 & \cellcolor{red!12}85.27 
    & \cellcolor{red!00}20.80 & \cellcolor{red!12}85.19 & \cellcolor{red!00}15.37 & \cellcolor{red!12}84.32 
    & \cellcolor{red!00}11.23 & \cellcolor{red!24}83.52
    \\
    Mistral 7b
    & \cellcolor{red!24}18.18 & \cellcolor{red!24}84.64 & \cellcolor{red!24}21.21 & \cellcolor{red!24}85.42
    & \cellcolor{red!24}22.52 & \cellcolor{red!24}85.33 & \cellcolor{red!24}16.86 & \cellcolor{red!24}84.45 
    & \cellcolor{red!24}12.35 & \cellcolor{red!24}83.52 
    \\
    Gemma1.1 7b
    & \cellcolor{red!00}15.94 & \cellcolor{red!00}82.85 & \cellcolor{red!00}18.92 & \cellcolor{red!00}84.47 
    & \cellcolor{red!00}20.19 & \cellcolor{red!00}84.51 & \cellcolor{red!00}14.93 & \cellcolor{red!00}83.32 
    & \cellcolor{red!00}10.89 & \cellcolor{red!00}81.51 
    \\
    Llama3.1 8b
    & \cellcolor{red!12}17.46 & \cellcolor{red!00}83.85 & \cellcolor{red!12}19.95 & \cellcolor{red!00}85.17
    & \cellcolor{red!12}21.30 & \cellcolor{red!00}85.06 & \cellcolor{red!12}16.19 & \cellcolor{red!00}84.19 
    & \cellcolor{red!12}11.75 & \cellcolor{red!12}82.31
    \\
    Llama3.1 70b
    & \cellcolor{red!00}17.06 & \cellcolor{red!00}83.48 & \cellcolor{red!00}19.24 & \cellcolor{red!00}83.30
    & \cellcolor{red!0}20.24 & \cellcolor{red!00}81.52 & \cellcolor{red!00}15.77 & \cellcolor{red!00}81.67
    & \cellcolor{red!00}11.60 & \cellcolor{red!00}78.78
    \\

    \midrule
    \multicolumn{11}{c}{Two-shot Setting} \\
    \midrule
        
    GPT-4o mini
    & \cellcolor{red!00}16.87 & \cellcolor{red!12}84.69 & \cellcolor{red!0}18.86 & \cellcolor{red!00}85.44 
    & \cellcolor{red!00}20.85 & \cellcolor{red!24}85.53 & \cellcolor{red!00}14.85 & \cellcolor{red!12}84.48 
    & \cellcolor{red!00}11.43 & \cellcolor{red!24}83.70
    \\
    Mistral 7b
    & \cellcolor{red!12}18.17 & \cellcolor{red!24}84.51 & \cellcolor{red!00}20.91 & \cellcolor{red!12}85.46
    & \cellcolor{red!00}22.92 & \cellcolor{red!00}85.31 & \cellcolor{red!12}16.82 & \cellcolor{red!24}84.50 
    & \cellcolor{red!00}12.31 & \cellcolor{red!12}83.63 
    \\
    Gemma1.1 7b
    & \cellcolor{red!00}16.46 & \cellcolor{red!00}83.19 & \cellcolor{red!00}18.72 & \cellcolor{red!00}84.94 
    & \cellcolor{red!00}20.54 & \cellcolor{red!00}84.28 & \cellcolor{red!00}14.47 & \cellcolor{red!00}83.73 
    & \cellcolor{red!00}11.11 & \cellcolor{red!00}82.21 
    \\
    Llama3.1 8b
    & \cellcolor{red!24}19.14 & \cellcolor{red!00}83.77 & \cellcolor{red!12}22.70 & \cellcolor{red!24}85.59
    & \cellcolor{red!24}24.13 & \cellcolor{red!12}85.43 & \cellcolor{red!00}16.60 & \cellcolor{red!00}84.16 
    & \cellcolor{red!12}12.46 & \cellcolor{red!00}82.71
    \\
    Llama3.1 70b
    & \cellcolor{red!00}20.69 & \cellcolor{red!00}79.85 & \cellcolor{red!24}26.20 & \cellcolor{red!00}85.43
    & \cellcolor{red!12}23.73 & \cellcolor{red!00}80.30 & \cellcolor{red!24}18.22 & \cellcolor{red!00}83.60
    & \cellcolor{red!24}13.45 & \cellcolor{red!00}82.87
    \\

    \midrule
    \multicolumn{11}{c}{Fine-tuning Setting} \\
    \midrule
    
    BART
    & \cellcolor{red!24}42.02 & \cellcolor{red!24}89.44 
    & \cellcolor{red!24}55.05 & \cellcolor{red!24}91.55 
    & \cellcolor{red!24}53.84 & \cellcolor{red!24}91.06 
    & \cellcolor{red!24}25.38 & \cellcolor{red!24}86.81 
    & \cellcolor{red!24}20.05 & \cellcolor{red!24}85.58 
    \\
    PEGASUS-X
    & \cellcolor{red!00}38.20 & \cellcolor{red!00}88.16 
    & \cellcolor{red!00}54.58 & \cellcolor{red!00}91.34 
    & \cellcolor{red!00}49.45 & \cellcolor{red!00}90.33 
    & \cellcolor{red!00}23.62 & \cellcolor{red!00}85.82 
    & \cellcolor{red!00}18.34 & \cellcolor{red!00}84.39 
    \\
    Llama3.1 8b
    & \cellcolor{red!00}20.55 & \cellcolor{red!00}85.27 
    & \cellcolor{red!00}29.20 & \cellcolor{red!00}86.84 
    & \cellcolor{red!00}33.91 & \cellcolor{red!00}87.70 
    & \cellcolor{red!00}16.33 & \cellcolor{red!00}83.60 
    & \cellcolor{red!00}10.66 & \cellcolor{red!00}82.70 
    \\
    
  

    \bottomrule

\end{tabular}}
\caption{Model performance based on style shift across five datasets, with evaluation metrics including BERTScore F1 and the geometric mean of ROUGE-1/2/L (ROUGE).}
\label{tab:2}
% \vspace{-1em}
\end{table*}


==> tables/topic_result.tex <==

% \begin{table*}[t!]
% \centering
% \setlength{\tabcolsep}{3pt}
% \resizebox{.99\textwidth}{!}{
% \begin{tabular}{l| cc|  cc| cc| cc| cc }
%     \toprule
%     \multirow{2}{*}{Model} & \multicolumn{2}{c|}{\textbf{Soccer}} & \multicolumn{2}{c|}{\textbf{Crime}} & \multicolumn{2}{c|}{\textbf{Family}} & \multicolumn{2}{c|}{\textbf{Media}} & \multicolumn{2}{c}{\textbf{Law}}   \\
%      & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore   \\
    
%     \midrule
% \multicolumn{11}{c}{Zero-shot Setting (Two-shot Setting)} \\
%     \midrule
    
%     GPT-4o mini
%     & \cellcolor{red!12}23.67 (-1.10) & \cellcolor{red!12}86.96 (-0.47)
%     & \cellcolor{red!00}26.90 (-6.22) & \cellcolor{red!24}87.92 (-4.32)
%     & \cellcolor{red!00}26.85 (-15.93) & \cellcolor{red!24}87.78 (-6.30)
%     & \cellcolor{red!00}22.08 (+2.94) & \cellcolor{red!12}86.95 (+2.39)
%     & \cellcolor{red!00}27.77 (-12.51) & \cellcolor{red!24}87.95 (-4.75)
%     \\
%     Mistral 7b
%     & \cellcolor{red!00}23.19 (-1.64) & \cellcolor{red!00}81.58 (-5.45)
%     & \cellcolor{red!00}26.17 (+1.02) & \cellcolor{red!00}83.86 (-3.85)
%     & \cellcolor{red!00}23.16 (-3.77) & \cellcolor{red!00}87.04 (+0.52)
%     & \cellcolor{red!12}22.96 (-1.42) & \cellcolor{red!00}85.29 (+4.05)
%     & \cellcolor{red!00}27.34 (-0.60) & \cellcolor{red!00}86.25 (-1.45)
%     \\
%     Gemma1.1 7b
%     & \cellcolor{red!00}23.65 (+0.08) & \cellcolor{red!00}86.07 (+0.40)
%     & \cellcolor{red!00}25.89 (-0.11) & \cellcolor{red!00}86.80 (+0.35)
%     & \cellcolor{red!00}25.06 (-0.74) & \cellcolor{red!00}86.52 (+0.23)
%     & \cellcolor{red!00}21.10 (-0.37) & \cellcolor{red!00}85.90 (+0.49)
%     & \cellcolor{red!00}25.53 (-0.05) & \cellcolor{red!00}86.53 (+0.26)
%     \\
%     Llama3.1 8b
%     & \cellcolor{red!24}25.06 (-1.07) & \cellcolor{red!24}87.01 (-0.18)
%     & \cellcolor{red!24}27.95 (-1.22) & \cellcolor{red!12}87.83 (-0.13)
%     & \cellcolor{red!12}27.80 (-0.29) & \cellcolor{red!12}87.71 (-0.61)
%     & \cellcolor{red!24}23.28 (-0.60) & \cellcolor{red!24}86.98 (-0.09)
%     & \cellcolor{red!12}28.48 (-0.75) & \cellcolor{red!12}87.86 (-1.37)
%     \\
%     Llama3.1 70b
%     & \cellcolor{red!00}24.53 (-0.12) & \cellcolor{red!00}84.65 (+3.32)
%     & \cellcolor{red!12}27.33 (-1.48) & \cellcolor{red!00}84.89 (+0.32)
%     & \cellcolor{red!24}28.31 (-0.45) & \cellcolor{red!00}87.10 (-0.01)
%     & \cellcolor{red!00}21.73 (+2.06) & \cellcolor{red!00}83.71 (+1.14)
%     & \cellcolor{red!24}28.59 (-1.01) & \cellcolor{red!00}87.75 (+0.26)
%     \\






    
    
%     \midrule
%     \multicolumn{11}{c}{Fine-tuning Setting} \\
%     \midrule
    
%     BART
%     & \cellcolor{red!24}29.71 & \cellcolor{red!24}88.90 
%     & \cellcolor{red!24}31.45 & \cellcolor{red!24}88.98
%     & \cellcolor{red!24}30.45 & \cellcolor{red!24}88.67 
%     & \cellcolor{red!24}27.56 & \cellcolor{red!24}88.20 
%     & \cellcolor{red!24}31.50 & \cellcolor{red!24}88.86 
%     \\
%     PEGASUS-X
%     & \cellcolor{red!00}24.74 & \cellcolor{red!00}87.79 
%     & \cellcolor{red!00}27.32 & \cellcolor{red!00}88.09 
%     & \cellcolor{red!00}27.00 & \cellcolor{red!00}87.89
%     & \cellcolor{red!00}24.12 & \cellcolor{red!00}87.54 
%     & \cellcolor{red!00}28.17 & \cellcolor{red!00}88.19 
%     \\
%     Llama3.1 8b
%     & \cellcolor{red!00}23.13 & \cellcolor{red!00}85.98 
%     & \cellcolor{red!00}28.18 & \cellcolor{red!00}87.39 
%     & \cellcolor{red!00}24.35 & \cellcolor{red!00}85.72 
%     & \cellcolor{red!00}23.11 & \cellcolor{red!00}85.71 
%     & \cellcolor{red!00}27.39 & \cellcolor{red!00}87.10 
%     \\
    
  

%     \bottomrule

% \end{tabular}}
% \caption{Model performance based on topic shift across five datasets, with evaluation metrics including BERTScore F1 and the geometric mean of ROUGE-1/2/L (ROUGE). Parenthetical values represent the performance gains or losses observed when comparing two-shot prompting to zero-shot prompting.}
% \label{tab:3}
% % \vspace{-1em}
% \end{table*}

\begin{table*}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{.99\textwidth}{!}{
\begin{tabular}{l| cc|  cc| cc| cc| cc }
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{2}{c|}{\textbf{Soccer}} & \multicolumn{2}{c|}{\textbf{Crime}} & \multicolumn{2}{c|}{\textbf{Family}} & \multicolumn{2}{c|}{\textbf{Media}} & \multicolumn{2}{c}{\textbf{Law}}   \\
     & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore & ROUGE & BERTScore   \\
    
    \midrule
    \multicolumn{11}{c}{Zero-shot Setting} \\
    \midrule
    
    GPT-4o mini
    & \cellcolor{red!12}23.67 & \cellcolor{red!12}86.96
    & \cellcolor{red!00}26.90 & \cellcolor{red!24}87.92
    & \cellcolor{red!00}26.85 & \cellcolor{red!24}87.78
    & \cellcolor{red!00}22.08 & \cellcolor{red!12}86.95
    & \cellcolor{red!00}27.77 & \cellcolor{red!24}87.95
    \\
    Mistral 7b
    & \cellcolor{red!00}23.19 & \cellcolor{red!00}81.58
    & \cellcolor{red!00}26.17 & \cellcolor{red!00}83.86
    & \cellcolor{red!00}23.16 & \cellcolor{red!00}87.04
    & \cellcolor{red!12}22.96 & \cellcolor{red!00}85.29
    & \cellcolor{red!00}27.34 & \cellcolor{red!00}86.25
    \\
    Gemma1.1 7b
    & \cellcolor{red!00}23.65 & \cellcolor{red!00}86.07
    & \cellcolor{red!00}25.89 & \cellcolor{red!00}86.80
    & \cellcolor{red!00}25.06 & \cellcolor{red!00}86.52
    & \cellcolor{red!00}21.10 & \cellcolor{red!00}85.90
    & \cellcolor{red!00}25.53 & \cellcolor{red!00}86.53
    \\
    Llama3.1 8b
    & \cellcolor{red!24}25.06 & \cellcolor{red!24}87.01
    & \cellcolor{red!24}27.95 & \cellcolor{red!12}87.83
    & \cellcolor{red!12}27.80 & \cellcolor{red!12}87.71
    & \cellcolor{red!24}23.28 & \cellcolor{red!24}86.98
    & \cellcolor{red!12}28.48 & \cellcolor{red!12}87.86
    \\
    Llama3.1 70b
    & \cellcolor{red!00}24.53 & \cellcolor{red!00}84.65
    & \cellcolor{red!12}27.33 & \cellcolor{red!00}84.89
    & \cellcolor{red!24}28.31 & \cellcolor{red!00}87.10
    & \cellcolor{red!00}21.73 & \cellcolor{red!00}83.71
    & \cellcolor{red!24}28.59 & \cellcolor{red!00}87.75
    \\

    \midrule
    \multicolumn{11}{c}{Two-shot Setting} \\
    \midrule
    
    GPT-4o mini
    & \cellcolor{red!00}22.57 & \cellcolor{red!00}86.49
    & \cellcolor{red!00}20.68 & \cellcolor{red!00}83.60
    & \cellcolor{red!00}24.92 & \cellcolor{red!24}87.70
    & \cellcolor{red!00}20.94 & \cellcolor{red!12}86.97
    & \cellcolor{red!00}25.92 & \cellcolor{red!24}87.98
    \\
    Mistral 7b
    & \cellcolor{red!12}24.83 & \cellcolor{red!12}87.03
    & \cellcolor{red!00}27.19 & \cellcolor{red!00}87.71
    & \cellcolor{red!00}26.93 & \cellcolor{red!12}87.56
    & \cellcolor{red!00}21.54 & \cellcolor{red!00}81.24
    & \cellcolor{red!00}27.94 & \cellcolor{red!00}87.70
    \\
    Gemma1.1 7b
    & \cellcolor{red!00}23.73 & \cellcolor{red!00}86.47
    & \cellcolor{red!00}25.78 & \cellcolor{red!00}87.15 
    & \cellcolor{red!00}24.32 & \cellcolor{red!00}86.75
    & \cellcolor{red!00}20.73 & \cellcolor{red!00}86.39
    & \cellcolor{red!00}25.48 & \cellcolor{red!00}86.79
    \\
    Llama3.1 8b
    & \cellcolor{red!24}26.13 & \cellcolor{red!24}87.19
    & \cellcolor{red!24}29.17 & \cellcolor{red!12}87.96
    & \cellcolor{red!12}28.09 & \cellcolor{red!24}87.70
    & \cellcolor{red!24}23.88 & \cellcolor{red!24}87.08
    & \cellcolor{red!24}29.23 & \cellcolor{red!12}87.88
    \\
    Llama3.1 70b
    & \cellcolor{red!00}24.53 & \cellcolor{red!00}84.65
    & \cellcolor{red!12}27.33 & \cellcolor{red!24}84.89
    & \cellcolor{red!24}28.31 & \cellcolor{red!00}87.10
    & \cellcolor{red!12}21.73 & \cellcolor{red!00}83.71
    & \cellcolor{red!12}28.59 & \cellcolor{red!00}87.75
    \\
    \midrule
    \multicolumn{11}{c}{Fine-tuning Setting} \\
    \midrule
    
    BART
    & \cellcolor{red!24}29.71 & \cellcolor{red!24}88.90 
    & \cellcolor{red!24}31.45 & \cellcolor{red!24}88.98
    & \cellcolor{red!24}30.45 & \cellcolor{red!24}88.67 
    & \cellcolor{red!24}27.56 & \cellcolor{red!24}88.20 
    & \cellcolor{red!24}31.50 & \cellcolor{red!24}88.86 
    \\
    PEGASUS-X
    & \cellcolor{red!00}24.74 & \cellcolor{red!00}87.79 
    & \cellcolor{red!00}27.32 & \cellcolor{red!00}88.09 
    & \cellcolor{red!00}27.00 & \cellcolor{red!00}87.89
    & \cellcolor{red!00}24.12 & \cellcolor{red!00}87.54 
    & \cellcolor{red!00}28.17 & \cellcolor{red!00}88.19 
    \\
    Llama3.1 8b
    & \cellcolor{red!00}23.13 & \cellcolor{red!00}85.98 
    & \cellcolor{red!00}28.18 & \cellcolor{red!00}87.39 
    & \cellcolor{red!00}24.35 & \cellcolor{red!00}85.72 
    & \cellcolor{red!00}23.11 & \cellcolor{red!00}85.71 
    & \cellcolor{red!00}27.39 & \cellcolor{red!00}87.10 
    \\
    
  

    \bottomrule

\end{tabular}}
\caption{Model performance based on topic shift across five datasets, with evaluation metrics including BERTScore F1 and the geometric mean of ROUGE-1/2/L (ROUGE).}
\label{tab:3}
% \vspace{-1em}
\end{table*}


